DEDUCE: Diverse scEne Detection methods in Unseen Challenging Environments

In recent years, there has been a rapid increase in the number of service robots deployed for aiding people in their daily activities. Unfortunately, most of these robots require human input for training in order to do tasks in indoor environments. Successful domestic navigation often requires access to semantic information about the environment, which can be learned without human guidance. In this paper, we propose a set of DEDUCE - Diverse scEne Detection methods in Unseen Challenging Environments algorithms which incorporate deep fusion models derived from scene recognition systems and object detectors. The five methods described here have been evaluated on several popular recent image datasets, as well as real-world videos acquired through multiple mobile platforms. The final results show an improvement over the existing state-of-the-art visual place recognition systems.

==> images/map_atkinson6th.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.15\textwidth]{images/ucsd_atkinson_6f_iros2019_fx_d.pdf}
  \caption{\small Semantic Map of the Contextual Robotics Institute building.  Each color represents one of the seven classes of the visual place categorization that our system classified.}
  \label{maps:atkinson}
\end{figure}

==> images/map_cse2.tex <==
\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.3\textwidth]{images/ucsd_cse_floor02_iros2019_vpc02.pdf}
  \caption{\small Semantic Map of the Computer Science and Engineering Department building.  Each color represents one of the seven classes of the visual place categorization that our system classified. }
  \label{map:cse}
\end{figure}
